How Segregation Patterns Affect the Availability of Fair District Plans

We create 4200 synthetic cities which vary in percent minority population and their residential segregation patterns. Of these, 1200 are modeled on existing cities, and 3000 are rectangular grid cities. In each city, we consider single-member voting district plans for a hypothetical city council election. A fair district plan is defined as one where the number of minority-majority districts is proportional to the city-wide minority population. Thus each city is summarized by three traits: minority percent, a measure of segregation, and availability of a fair district plan. We find that when the minority population is around 25%-33%, there is a positive correlation between the degree of segregation and the availability of proportional district plan. Consistently, when the minority population lives in a more diffuse residential pattern, there are fewer available proportional district plans. Finally, we develop a new method to validate runtime and sample size of an ensemble of district plans created by the GerryChain software program.

==> blkarray/blkarray.tex <==
\AtBeginDocument{\date{27 February 2015}}
\input{blkarray.sty}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


